Invariant Grounding for Video Question Answering

Video Question Answering (VideoQA) is the task of answering questions about a video. At its core is understanding the alignments between visual scenes in video and linguistic semantics in question to yield the answer. In leading VideoQA models, the typical learning objective, empirical risk minimization (ERM), latches on superficial correlations between video-question pairs and answers as the alignments. However, ERM can be problematic, because it tends to over-exploit the spurious correlations between question-irrelevant scenes and answers, instead of inspecting the causal effect of question-critical scenes. As a result, the VideoQA models suffer from unreliable reasoning. In this work, we first take a causal look at VideoQA and argue that invariant grounding is the key to ruling out the spurious correlations. Towards this end, we propose a new learning framework, Invariant Grounding for VideoQA (IGV), to ground the question-critical scene, whose causal relations with answers are invariant across different interventions on the complement. With IGV, the VideoQA models are forced to shield the answering process from the negative influence of spurious correlations, which significantly improves the reasoning ability. Experiments on three benchmark datasets validate the superiority of IGV in terms of accuracy, visual explainability, and generalization ability over the leading baselines.

==> sec/3_method.tex <==
% \section{Method}
% Under a causal look of the video-generating process, we formalize the principle of our invariant grounding framework. Throughout the paper, upper-cased letters like $V$ denote random variables, while lower-case letters like $v$ denote the deterministic value of variables.

% \subsection{Causal View of VideoQA}
% \label{sec:causal-view}
% % depict our SCM
% Prediction with transparency requires understanding the actual mechanisms of the task of interest.
% Here we formalize the causal view for VideoQA tasks by using a Structure Causal Model (SCM) \cite{10.5555/1642718, alma991011292629705181} with variables of four: input video $V$, given $Q$, context scene $T$, critical scene $C$ and ground-truth answer$A$.  Figure \ref{fig:scm} illustrates the SCM, where each link denotes a causal relationship between two variables. 
% \begin{itemize}[leftmargin=*]
% \setlength\itemsep{-.3em}
% \item $C\gets V\to T$ The input video V consists of two parts C and T. For example, the input video in Figure \ref{fig:runing_example}(a) is disjoint into the first two shots and the last three shots, which are the context and critic scene respectively.
% \item $V\to C\gets Q$ The critic scene C is conditional upon input video V and question Q. For a given V, variation in Q can produce C with other content.
% \item $Q\to A\gets C$ 
% For given $Q$, the “critical frames” means $C$ is the only endogenous parent to determine the ground truth answer $A$. Taking the example in Figure \ref{fig:runing_example}(a) again, $C$ denotes the oracle rationale that perfectly explains why the \textit{jump} is labeled as ground-truth. 
% \item $T\dashleftarrow\dashrightarrow C$ This dashed arrow indicates additional probabilistic dependencies \cite{10.5555/1642718,reason:Pearl09a} between $C$ and $T$. Given input $Q,V$ We consider three typical relationships here: 1) $C$ is independent of $T$ (\textit{i.e.,} $T \bot C \parallel Q,V$); 2) $C$ is the direct cause of $T$, or vise versa (\textit{i.e.,} $T \rightleftharpoons  C \parallel Q,V$; and 3) There exists a common cause $E$ (\textit{i.e.,} $T \gets E\to  C \parallel Q,V$. See Appendix or the corresponding examples. 
% \end{itemize}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=1\linewidth]{fig/scm.pdf}
%     \vspace{-5pt}
%     \caption{Figure 1. (a) Causal view of VideoQA; (b) Illustration of interventional distribution}
%     \label{fig:scm}
%     \vspace{-15pt}
% \end{figure}



% %back doors in our SCM
% In the light of our SCM, VideoQA models suffer from the spurious correlation between the background frame $T$ and the ground-truth answer $A$ via multiple shortcuts. Inevitably, the existence of $Q$ and $V$ naturally confounded backdoor path $T \gets V \to C \to A$ and $T \gets V \to C \gets Q \to A$. 
% To make the matter worse, $T\dashleftarrow\dashrightarrow C$ further amplified this issue. Assuming $C \to T$,  $C$ serves as confounder between $T$ and $A$ , which opens a backdoor path $T \gets C \to A$, 
% thus making $T$ and $A$ spuriously correlated \cite{reason:Pearl09a}.
% % We systematize such spurious correlations as $A\not\!\bot T$, where $\bot$ denotes probabilistic independence. 
% Furthermore, data collected from different environments exhibit various spurious correlations \cite{DBLP:journals/corr/abs-2002-11894,arjovsky2020invariant}, e.g., one mostly picks video with person race on the track as the training data, while another selects video with person jump across the track as the testing data. Hence, such spurious shortcuts enforced via $T$ are unstable and variant across different distributions. 

% \subsection{Task Formalization}
% \noindent\textbf{VideQA Definition}
% % general defination of VideoQA
% Given a Video $V$ and a question $Q$, VideoQA aims to predict the correct answer $\hat{a}$ relevant to the visual content:
% \begin{equation}\label{eq1}
%     \hat{a} = \argmax_{a \in \mathcal{A}} h(a\mid Q,V)
% \end{equation}
% where $\mathcal{A}$ is answer space and $\mathcal{h}$ is the mapping function. 
% Similar to the previous works \cite{jiang2020reasoning,le2021hierarchical}, we represent a video with $K$ shots as $V^{K\times d_v}=\left \{ v_{k}^{d_v} \right \}_{k=1}^{K}$, a language query of length $L$ as $Q^{L\times d_q}=\left \{ q_{l}^{d_q} \right \}_{l=1}^{L}$, where $d_v$ and $d_q$ are the hidden space for visual and language representation.

% % Existing work use ERM
% Existing work \cite{fan2019heterogeneous,gao2018motionappearance,le2021hierarchical,jiang2020reasoning,Jiang_Chen_Lin_Zhao_Gao_2020} implement Equation \ref{eq1} by minimizing the empirical risk:
% \begin{equation}\label{eq2}
%     \min_{h} \mathcal{R}(h(Q,V),\:A)
% \end{equation}
% where $\mathcal{R}$ is the risk function in form of cross-entropy loss or hinge loss. Nevertheless, this learning strategy relies heavily on the statistical associations between the input features and labels, and can potentially exhibit non-causal prediction.

% \noindent\textbf{Invariant Rationale in IGV}
% With reference to the causal theory \cite{reason:Pearl09a,10.5555/1642718}, for each variable $X$ in a SCM, there exists a directed link from each of its parent variables $PA(X)$ to $X$, if and only if the causal mechanism $X = f_x(PA(X),\epsilon_X)$ persists, where $\epsilon_X \bot PA(X)$ is the exogenous noise of X. 
% For simplicity, we omit the exogenous noise and simplify it as $X = f_x(PA(X))$. 
% Hence, there exist a function $f_A:C,Q\to A$ in our SCM, where the “oracle rationale” $C$ satisfies:
% \begin{equation}\label{eq3}
%     A=h(C,Q), \;\;\;  A\bot T \mid C,Q
% \end{equation}

% However, in fact, only the pairs of input $V,Q$ and label $A$ are observed during training, while neither oracle rationale $C$ nor oracle structural equation model $h$ is accessible. 
% Such an absence of oracles calls for the study on introspective evidence.
% In view of our SCM, we systematize an intrinsically-interpretable framework as a combination of two modules $h_{\hat{A}} \, \circ\, h_{\tilde{C}}$. That is, $h(V, Q)=h_{\hat{A}}\,\circ \,h_{\tilde{C}}(V, Q)$, where $h_{\tilde{C}}$ discovers critic frames $C$ from the observed $Q$ and $V$, and $h_{\hat{A}}$ outputs the prediction $\hat{A}$ to approach $A$. 
% Distinct from $C$ and $A$ which are the variables in the causal mechanisms, $\tilde{C}$ and $\hat{A}$  denote their approximation in the modeling process.

% We ascribe the fore-mentioned limitation of existing work (\textit{i.e.}, Equation \ref{eq2}) to ignoring $A\bot T \mid C,Q$ in Equation \ref{eq3}, which is crucial to refine the causal relationship $C \to A$, that is invariant across different $T$. By introducing this independence, we formalize the gist of invariant grounding as:
% \begin{equation}\label{eq4}
%       \min_{h_{\tilde{C}},h_{\hat{A}}} \mathcal{R}(h_{\hat{A}}\circ h_{\tilde{C}}(V, Q),\:A), \;\;\;\; \text{s.t.}\;A\bot \tilde{T}\mid\tilde{C},Q
% \end{equation}
% where $\tilde{T}={V}\backslash \tilde{C}$ is the complement of $\tilde{C}$. This formulation encourages the rationale $\tilde{C}$ seeking the patterns that are stable across different distributions, while discarding the unstable patterns.
 
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{fig/overview.pdf}
    \vspace{-5pt}
    \caption{Overview of our IGV framework.}
    \label{fig:overview}
    \vspace{-15pt}
\end{figure}

%\subsection{Data Representation} 
% 我看VideoQA 很多都有这节，是否必要？
%\noindent\textbf{Video Representation}.
%\noindent\textbf{Question Representation}. 


\subsection{IGV Learning Strategy}
To reflect the insight of \ref{eq4}, IGV with intrinsic interpretability is designed with two modules $h=h_{\hat{A}}\,\circ\,h_{\tilde{C}}$, where $h_{\tilde{C}}$ is to extract critic scene, and $h_{\hat{A}}$ is to make prediction based on the critic scene. 

Fig \ref{fig:overview} shows our framework in a nutshell. Conditioned on input $Q$, a grounding indicator first split the video into critical scene and context,
then a scene intervener spoils the context part by replacing it with substituted sampled from the memory bank. Hereafter, coupled with textual information, the causal, context, and intervened scenes are fed into the backbone predictor to create three cross-modal representations, which are further projected to answer space.


% \subsubsection{Grounding Indicator}
% %这里实现我用的是两个attention 实现，但现在觉得一个att更合理
% % 根据是否需要描述Gumbel的过程，我写了两个版本
% % 1，描述Gumbel
% % To establish $h_{\tilde{C}}$ that 
% To recover the oracle rationale $C$ from the joint distribution over the inputs and labels. Two independent Long short-term memory (LSTM) are adopted to encode visual and linguistic features separately. Based on their output, a question-guided grounding indicator learns a  normalized attention scores $ S_1, \in \left\{ 0\sim 1 \right\}^{K} $ for each of $K$ shot in the $V$, where $S_{k,1}$, $S_{K,0}=1-S_{k,1}$ indicates the probability of shot $v_k$ of being a critical scene and context, respectively:
% \begin{equation}\label{v-encoder}
%     V_g, V_l=\text{LSTM}_V(V), \;\; Q_g, Q_l=\text{LSTM}_Q(Q)
% \end{equation}
% \begin{equation}\label{eq5}
%     S_1=\text{Softmax}(Q_gV_{l}^{T})%, \; for\; i \in \left\{ C,T \right\}
% \end{equation}
% where outputs $Q_l \in \mathbb{R}^{L \times d}$, $V_g\in \mathbb{R}^{ K \times d}$ are the local representation of $Q$ and $V$, the last hidden state $Q_g$,$V_g$ denote their global representations, $d$ is the hidden dimension. 

% Hereby, the process of grounding attribution $I \in \left\{ 0,1 \right\}^{K\times2}$  essentially follows $I_k \sim \text{Bernoulli}(S_1)$ for each shot. 
% However, sampling from discrete distribution makes the network non-differentiable. To make grounding indicator end-to-end trainable, we apply the Gumbel-Max trick and smooth the sampling process as:
% \begin{equation}\label{eq6}
%     I_{k}=\argmax_{i \in \left\{ 0,1 \right\}}({\log{S_{k,i}}+g_i})
% \end{equation}
% where $g_{i}=-\log(-\log(u_i)$ denotes the Gumbel noise and $u_i$ is i.i.d. sampled from \textit{Uniform}(0,1). We can further relax the non-differentiable operation \textit{argmax} in Equation \ref{eq6} with \textit{softmax} as: 
% \begin{equation}
% \begin{split}\label{eq7}
%     I_k=\left\{ S_{k,i} \mid S_{k,i}=  \frac{\exp((\log{S_{k,i}+g_i})/\tau)}{\sum_{j=0}^{1}\exp((\log{S_{k,j}+g_j})/\tau)}  \right\}, \\for \;i\in\left\{ 0,1 \right\}
% \end{split}
% \end{equation}
% with low temperature $\tau$, the sampling approximates the \textit{argmax} operation in Equation \ref{eq6} that enact over all pairs of $S_{k,1}$ and its counterpart $S_{k,0}$. Signified with scene indicator $I$ whose two dimensions respectively masks critical scene and context, we can acquire visual expression of $C \in \mathbb{R}^{N\times d_v}$ and $T \in \mathbb{R}^{(K-N)\times d_v}$ by assembling $V$ with $S_{1}$ and $S_{0}$, accordingly,
% % \begin{equation}\label{eq8}
% %     C=\text{E}_{C}(V, S_{1}),\;\;T=\text{E}_{T}(V, S_{0})
% % \end{equation}
% where $N\le K$ is the number of critical scene.
% % $\text{E}_{C}$ and $\text{E}_{T}$ are visual encoders for causal and trivial scene, respectively.

% % % %2，不介绍gumbel 的过程
% % \lyc {recover the oracle rationale $C$ from the joint distribution over the inputs and labels, a question-guided grounding indicator first learns  a  normalized attention scores $ S, \in \left\{ 0\sim 1 \right\}^{K} $ for each of $K$ shot in the $V \in\mathbb{R}^{K\times d}$, where $S_{k}$ indicates the probability of shot $v_k$ of being a critical scene and context, respectively:
% % \begin{equation}\label{eq5}
% %     S=\text{Softmax}(Q_gV^{T})
% % \end{equation}
% % where $Q_g \in \mathbb{R}^{d}$ is the global representation of $Q$.Then, to decide the grounding attribution for each shot, which is essentially discrete operations, we apply the Gumbel-Max trick [9] with low temperature ($\tau$=0.9) to approximates the $\argmax$ operation over all pairs of $S_k$ and its counterpart $1-S_k$:
% % \begin{equation}\label{eq6}
% %     I_k=\argmax{\left\{S_k, 1-S_k\right\}}
% % \end{equation}}


% % Attention + Gumbel
% \subsubsection{Scene Intervener}
% \label{section:si}
% The scarcity of shot-level supervision incapacitates grounding indicator to modeling $h_{\tilde{C}}$ alone. To remedy this issue, scene intervener is devised as an auxiliary module to strengthen the functionality of grounding indicator by constructing different environment $M \in \mathbb{R}^{K \times d_v}$ to infer the invariant features.

% Concretely, On the top of our SCM, we generate t-interventional distribution by conducting intervention $do(T = t)$ on the trivial scene, 
% % and fixes S to the specific value s.  
% It first collect $\tilde{t}$ as video shots in training set into a memory bank $\mathbb{\tilde{T}} = \left\{ \tilde{t} \right\}$. Next, according to $I_0$, it samples a dummy $\tilde{t_i} \in \mathbb{\tilde{T}}$ to perform $do(T = \tilde{t_i})$ --- replacing the context scene $\tilde{t_j}$ and construct a intervened video $\tilde{m}$ as $(\tilde{c}_j,\tilde{t}_i)$, where $i$, $j$ are indices. 

% Distinct from existing invariant learning work that partition the training set by prior knowledge \cite{arjovsky2020invariant, REx, DBLP:conf/icml/ChangZYJ20}, our scene intervener does not assume prophets about environments but introduces the interventional distribution 
% % \cite{DBLP:conf/aaai/TianKP06, pearl2016causal} 
% instead. Such construction of environment helps to distill the salient features as invariance that are consistently informative and uniform across these environments. 
% % Consequently, the scene intervener serves to remove the impact of shortcut learning by dismissing every link from the parents $PA(T)$ to the $T$. 

\subsubsection{Backbone Predictor}
Most VideoQA architectures from the state of the art are compatible with our IGV learning strategy. To testify, we design a simple and effective architecture inspired by \cite{jiang2020reasoning}. Specifically, $h_{\tilde{A}}$ is presented as a combination of a visual-question mixer and an answer decoder. The mixer first encode $\tilde{c}$:
\begin{equation}
    \tilde{C}_g, \tilde{C}_l=\text{LSTM}(\tilde{c})
\end{equation}
where outputs $\tilde{C}_g \in \mathbb{R}^{d}$, $\tilde{C}_l \in \mathbb{R}^{N \times d}$ denote the global and local feature of $\tilde{c}$ respectively. Then, based on the concatenation of local representation $Q_l$ and $V_l$, we construct an undirected heterogeneous graph that propagates information over each video shot and each question token. Typically, the adjacency matrix $G_{\tilde{c}} \in \mathbb{R}^{(L+N)\times (L+N)}$ is computed as the node-wise correlation scores in form of dot-product similarity. The output of the graph is combines them as holistic local factor $S_{\tilde{c}}^l \in \mathbb{R}^{d}$ via a attention pooling operator.
% Upon the acquisition of GCN output, attention pooling is , 
More Formally, the process is as follows: 
\begin{equation}
    X_{\tilde{c}}=\left[Q_l;\tilde{C}_l \right], \; G_{\tilde{c}}=\Phi_1(X_{\tilde{c}})\Phi_2(X_{\tilde{c}})
\end{equation}
\begin{equation}
    Z_{\tilde{c}}=\text{GCN}(X_{\tilde{c}}, G_{\tilde{c}})
\end{equation}
\begin{equation}
    S_{\tilde{c}}^l=\text{Pooling}(Z_{\tilde{c}})
\end{equation}
where $X_{\tilde{c}}$,$Z_{\tilde{c}} \in \mathbb{R}^{(L+N)\times d}$ 
denote the input and output of graph reasoning, $\Phi_1$ and $\Phi_2$ denote affine projection followed by non-linear activation. 

To capture the global information, our mixer integrates two global factors $\tilde{C}_g$ and $Q_g$ into holistic representation via \textit{Block} fusion \cite{BenYounes_2019_AAAI}:
\begin{equation}
    S_{\tilde{c}}^g=\text{Block}(\tilde{C}_g,Q_g)
\end{equation}
Similarly, we obtain the final representation by applying the \textit{Block} again to global and local factor, which is further decoded into answer space with classifier $\Psi$:
\begin{equation}
    H_{\tilde{c}}=\text{Block}(S_{\tilde{c}}^g,S_{\tilde{c}}^l)
\end{equation}
\begin{equation}
    \hat{y}_{\tilde{c}}=\Psi(H_{\tilde{c}})
\end{equation}

Analogously, we can obtain $\hat{y}_{\tilde{t}}$ for $\tilde{t}$ and $\hat{y}_{\tilde{m}}$ for $\tilde{m}$ via the shared predictor. $\hat{y}_{\tilde{c}}$, $\hat{y}_{\tilde{t}}$ is the prediction based merely on the critical scene and context, while $\hat{y}_{\tilde{m}}$
measures the predictive power of intervened scene $\tilde{m}$. 

\subsection{Training Objective} 
To identify a critic scene C whose relationship with the answer A is stable across different distribution, we propose the IGV principle of invariant grounding applies if an model $h$ simultaneously minimize:
\begin{itemize}
    \item [1.] invariant risk: $\mathbb{E}_{c}\left[ \mathcal{R}(h(Q,C),A)\mid C=c \right]$
    \item [2.]  t-interventional risk: 
    $\mathbb{E}_{M}\left[ \mathcal{R}(h(Q,M),h(Q,C))\mid M=m, C=c \right]$
    \item [3.] context risk: $\mathbb{E}_{T}\left[ \mathcal{R}(h(Q,T), Uniform) \mid T=t \right]$
\end{itemize}
In general, the principle 1 and 2 are underpinned by  facts that variant feature mined in $C$ is sufficient and necessary to infer unbiased $\hat{A}$, and not affected by variation in T.  The principle 3 implies context should be uninformative.
% \subsubsection{Joint Learning Procedure}/

\noindent\textbf{training}.
Guided by the proposed principle, we design the learning objective as:
\begin{equation}
\begin{aligned} 
    \mathcal{L}_{IGV}=\text{XE}(h(Q,\tilde{c}),A)\,+\,\lambda_1\text{KL}(h(Q,\tilde{m}),h(Q,\tilde{c}))\\ \,+\,\lambda_2\text{KL}(h(Q,\tilde{m}),Uniform)
\end{aligned} 
\end{equation}
where XE and KL denote cross-entropy loss and KL-divergence, $\lambda_1$ and $\lambda_2$ are hyper-parameters.

By making the distribution-relevant risks indifferent while pursuing low risks, the IGV principle is able to discover the critic scene $\tilde{C}$ as the approximation of the oracle rationales $C$, while encouraging $h_{\tilde{A}}$ approaching the oracle model.

\noindent\textbf{Inference}. 
In the inference phase, we yield $y_{\tilde{c}}$ as the casual prediction that exclude the influence of the context $\tilde{t}$.
% \subsubsection{Answer Decoder}
% \noindent\textbf{Open-Set}.

% \noindent\textbf{Multi-choice}.



==> sec/7_limitation.tex <==
\section{Limitations}
\label{section:limits}
\lyc{In addition to technical advantages, we discuss the inadequacy in this section, whose refinement shall further boost the performance. 1) Unlike existing SoTA (\eg HOSTR) that utilize the object-level feature, IVG merely exploits the power of clip-level feature. Although the architecture of backbone model is beyond the scope of this work, we anticipate fine-grained feature will strengthen current IGV design.
2) Current intervention strategy can possibly threaten the causal prediction by introducing context with new shortcuts. Since the scene intervener sample context stratification in a random manner, there is a slight chance to draw an undesired substitute that nested with strong static relation towards  a wrong answer, thus inducing a false prediction.}

==> sec/X_instructions.tex <==
% --- repeat the title (AT: haven't found a more elegant way to do this...)
\twocolumn[
\centering
\Large
\textbf{\LaTeX\ Author Guidelines for \confName~Proceedings (2022)}
\vspace{1.0em}
] %< twocolumn
\appendix

\setcounter{section}{0}
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of cvpr.sty to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the CVPR70 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.


% Update the cvpr.cls to do the following automatically.
% For this citation style, keep multiple citations in numerical (not
% chronological) order, so prefer \cite{Alpher03,Alpher02,Authors14} to
% \cite{Alpher02,Alpher03,Authors14}.


\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

%------------------------------------------------------------------------
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

%------------------------------------------------------------------------
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> tab/ablation-loss-rebuttal.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet3'
\setlength{\tabcolsep}{6.5pt}
\begin{table}[ht]
\small
  \centering
  \caption{Study of IGV loss components}
   \vspace{-10pt}
    \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{l|cc|cc}
    \toprule
    \multirow{2}[1]{*}{Variants} & \multicolumn{2}{c}{MSVD-QA} & \multicolumn{2}{c}{MSRVTT-QA} \\
          & Our Backbone   & Co-Mem \cite{gao2018motionappearance} & Our Backbone   & Co-Mem \cite{gao2018motionappearance} \\
    \midrule
    \midrule
    Baseline & 36.1  & 34.6  & 36.3  & 35.3 \\
    $\Lapl_{\hat{c}}$     & 36.0    & 33.3  & 36.7  & 36.0 \\
    $\Lapl_{\hat{c}}+\Lapl_{\hat{t}}$   & 37.4  & 36.1  & 37.8  & 36.8 \\
    $\Lapl_{\hat{c}}+\Lapl_{v^{*}}$   & 38.2  & 36.3  & 37.4  & 36.2 \\
    $\Lapl_{\hat{c}}+\Lapl_{\hat{t}}+\Lapl_{v^{*}}$ & \textbf{40.8} & \textbf{37.7} & \textbf{38.3} & \textbf{37.3} \\
    \bottomrule
    \end{tabular}
    }
  \label{tab:ablation-loss}%
  \vspace{-15pt}
\end{table}%




==> tab/tgif-rebuttal.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet3'
\setlength{\tabcolsep}{6.5pt}
\begin{table}[ht]
\small
  \centering
  \caption{Comparison of accuracy on TGIF-QA test set}
   \vspace{-11pt}
    \resizebox{0.65\columnwidth}{!}{
    \begin{tabular}{c|ccc}
    \toprule
    Models & Action & Trans & FrameQA \\
    \midrule
    \midrule
    HGA   & 75.4  & 81    & 55.1 \\
    B2A   & \underline{75.9}  & 82.6  & 57.5 \\
    HCRN  & 75    & 81.4  & 55.9 \\
    HOSTER & 75    & \underline{83}    & \underline{58} \\
    \midrule
    \midrule
    Our Backbone & 75.4  & 81.3  & 55.4 \\
    IGV   & \textbf{76.7}  & \textbf{84}  & \textbf{59.1} \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:tgif-qa}%
  \vspace{-20pt}
\end{table}%


